NaVILA: Legged Robot Vision-Language-Action Model for Navigation

This paper proposes to solve the problem of Vision-and-Language Navigation with legged robots, which not only provides a flexible way for humans to command but also allows the robot to navigate through more challenging and cluttered scenes. However, it is non-trivial to translate human language instructions all the way to low-level leg joint actions. We propose NaVILA, a 2-level framework that unifies a Vision-Language-Action model (VLA) with locomotion skills. Instead of directly predicting low-level actions from VLA, NaVILA first generates mid-level actions with spatial information in the form of language, (e.g., "moving forward 75cm"), which serves as an input for a visual locomotion RL policy for execution. NaVILA substantially improves previous approaches on existing benchmarks. The same advantages are demonstrated in our newly developed benchmarks with IsaacLab, featuring more realistic scenes, low-level controls, and real-world robot experiments. We show more results at https://navila-bot.github.io/

==> sections/03-Method.tex <==
\maketitle
\begin{figure}[t]
  \centering
  \includegraphics[width=1\textwidth]{images/overview/v1.pdf}
  \caption{\method is a two-level framework combining high-level visual language understanding with low-level locomotion control. Our VLA model processes single-view images to produce mid-level actions in natural language, which are then converted into precise joint movements by an advanced low-level locomotion policy. This integration allows for strong generalization and adaptability across different real-world environments, and can operate the robot in real-time.}
  \label{fig:overview}
  % \vspace{-10pt}
\end{figure}

\section{Method}
\label{sec:method}
Our VLA model (\method) integrates high-level visual language understanding and action with low-level locomotion control (Figure~\ref{fig:overview}). \method employs a VLM that processes single-view images to generate waypoint instructions in natural language. These instructions are then interpreted by a low-level locomotion policy, which translates them into precise joint movements for real-time robot control. The synergy between the VLM's high-level reasoning and the locomotion policy's execution capabilities enables our method to demonstrate remarkable generalization and adaptability across diverse real-world environments. In the following sections, we detail the components of our approach. We begin by describing how we tame VLMs for high-level VLN in Sec.~\ref{sec:method:high}, followed by an overview of our robot configuration and low-level locomotion policy in Sec.~\ref{sec:method:low}. 


\subsection{Taming VLMs for High-level Vision Language Navigation}
\label{sec:method:high}
VLN requires processing video inputs as observations. A common approach to handling video inputs in VLMs is through video encoders. However, recent progress in VLMs has largely been driven by the availability of image-text data. While there have been efforts to extend this success to video encoders, the lack of large, high-quality video-text datasets has limited their pre-training. To address this challenge, we opt for image-based vision-language models in our approach. These models exhibit stronger generalization abilities and possess broader knowledge, making them more suitable for tackling the generalization challenges in VLN. Specifically, we built our approach upon VILA~\citep{lin2024vila,wu2024vila,fang2024vila,xue2024longvila,ye2024x,huang2025lita}, a family of efficient VLMs for both understanding and generation. VILA's pre-training has proven particularly effective for multi-image reasoning, making it especially suitable for VLN tasks where understanding sequential image relationships is critical.

\myparagraph{VILA Preliminary.}
VILA consists of three main components: a vision encoder, a projector, and an LLM. The vision encoder processes the input images, converting them into a sequence of visual tokens. These tokens are then downsampled and mapped into the language domain via an MLP projector. Afterward, the projected tokens, along with text tokens, are sent to the LLM for auto-regressive generation. When handling videos, VILA uniformly sampled frames at regular intervals. It puts all the frame information before any text. A typical prompt for describing a video might look like ``\texttt{$\langle$frame3$\rangle$$\langle$frame6$\rangle$$\langle$frame9$\rangle$...Tell me about this video.}'' Notably, with sequence parallel training~\citep{xue2024longvila}, VILA can include frames up to 1024. VILA undergoes a 3-stage training process: first, it pre-trains a connector between the frozen LLM and vision backbones using alignment data~\citep{liu2023visual}; then it pre-trains both the connector and the LLM using text-image interleaved corpus~\citep{coyo,zhu2024multimodal}; and finally, it fine-tunes all modules (vision encoder, connector, LLM) with instruction tuning data~\citep{liu2023visual,liu2024improved}.


\myparagraph{Navigation Prompts.}
In vision-language navigation tasks, images from different time steps serve two distinct purposes. The image at time step $t$ represents the current observation, which is crucial for a VLN agent to make immediate decisions (e.g., turning right at an intersection or stopping when the goal is reached). On the other hand, frames before time step $t$ are historical frames that function as a memory bank, helping the agent track overall progress (e.g., remembering the starting location, reasoning about places already visited and planning the next step). Uniformly sampling frames at regular intervals, as done in VILA, is not ideal because it doesn't differentiate between these two types of representations. Therefore, we first extract the most recent frame $t$ as the current observation and then uniformly sample frames from the preceding $t-1$ frames, ensuring the first frame is always included. Additionally, since current and historical observations serve different roles, we distinguish them in our task prompt using textual cues like \texttt{a video of historical observations:} for memory frames and \texttt{current observation:} for the latest frame. Unlike~\citep{zhang2024navid}, we avoid introducing additional special tokens that could complicate the LLM's learning process. Instead, we adhere to our design principle of keeping both the input and output of LLM in the language domain to fully leverage the reasoning capabilities of the pre-trained LLM. By integrating these tokens for historical and current observations with the navigation instruction, we construct a navigation task prompt, as shown in Figure~\ref{fig:overview}.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.95\textwidth]{images/vlm_arch/VLM-arch.pdf}
  \caption{Overview of our VLA framework. We denote the purple blocks (\protect\scalerel*{\includegraphics{images/misc/purple.pdf}}{A}) as memory tokens sampled from historical frames, and the red blocks (\protect\scalerel*{\includegraphics{images/misc/red.pdf}}{A}) as the current observation tokens. \protect\scalerel*{\includegraphics{images/misc/cap_trainable.pdf}}{A} denotes trainable parameters. In our experiments, we tested configurations with 8 to 64 frames for $t$.}
  \label{fig:vlm-arch}
  % \vspace{-15pt}
\end{figure}

\myparagraph{Supervised Fine-tuning Data Blend.}
Effective Supervised Fine-tuning (SFT) data is crucial for developing a robust vision-language action model. Such a model should be specialized for an embodied task yet avoid overfitting to specific actions. It should also generalize well to real-world scenarios while retaining broad-world knowledge. Thanks to NaVILA's modular framework design, which offers exceptional scalability and adaptability, it is straightforward to integrate new data sources into our pipeline. This flexibility allows us to consider diverse data sources to improve generalizability for navigation. We designed our SFT data blend from four perspectives: (1) Navigational data from real videos, (2) Navigational data from simulations, (3) Auxiliary navigational data, and (4) General VQA datasets.



First, we incorporate navigational data from real human touring videos. Recent studies~\citep{guhur2021airbert,majumdar2020improving,lin2023learning} have shown that collecting trajectory-instruction pairs from internet-data helps with navigation in discrete settings. However, extending this approach to continuous settings has remained challenging due to the difficulty of obtaining continuous action labels. Recent advances in metric-pose estimation in the wild have now made this feasible. Our data pipeline, shown in Figure\ref{fig:data-pipeline}, starts with 2K egocentric touring videos from YouTube. These videos provide a rich source of real data to learn robot navigation from human behavior. We process them into 20K trajectories using entropy-based sampling~\citep{lin2023learning} to ensure variety and representativeness. Then, we estimate camera poses using Mast3R~\citep{leroy2024grounding} to extract step-by-step actions and generate natural language instructions for each trajectory using VLM~\citep{lin2024vila} captioning and LLM~\citep{openai2024gpt4o} rephrasing.




\begin{figure}[t]
  \centering
  \includegraphics[width=0.95\textwidth]{images/human_videos/pipeline.pdf}
  \caption{Data pipeline for transforming human touring videos in the wild into pairwise navigation data within a continuous environment. We begin by processing the videos into meaningful trajectories through entropy-based sampling~\citep{lin2023learning}. Then we extract step-wise actions through metric camera pose estimation~\citep{leroy2024grounding}, and utilize VLM~\citep{lin2024vila} and LLM~\citep{openai2024gpt4o} to generate instructions.}
  \label{fig:data-pipeline}
  % \vspace{-15pt}
\end{figure}


Second, we focus on navigational data in simulations. Currently, there are limited options for VLN datasets in continuous environments, with only R2R-CE~\citep{r2r} and RxR-CE~\citep{rxr} available. These datasets provide sparse path points converted from discrete VLN versions. We utilize both datasets within the Habitat simulator, employing a shortest path follower to generate action sequences that adhere to the geodesic shortest path. This results in step-wise navigation videos, where each sample in our dataset comprises a $t+1$ frames video and the corresponding oracle action at time step $t$. To encourage the LLM to generate continuous value labels for distances and angles, we merge consecutive actions (e.g., combining two forward 25 cm steps into a single forward 50 cm step), with a maximum of three consecutive actions. This merging process has two key advantages: it reduces the dataset size for more efficient processing, and it helps prevent overfitting by introducing greater diversity in the actions. Additionally, to address label imbalance, particularly the underrepresentation of the stop action, we apply a rebalancing technique for a more even distribution. For all navigation-specific data, we apply the previously described frame extraction strategy and navigation task prompt.


Third, to improve scene understanding and address the limited instructions in current R2R-CE and RxR-CE, we incorporate auxiliary navigational datasets. Following~\citep{zhang2024navid}, we use augmented instructions from EnvDrop~\citep{tan2019learning} and introduce an auxiliary task of navigation trajectory summarization. Specifically, given a trajectory video, we sample frames by retaining the first frame and uniformly sampling the remaining ones as historical frames, and use the annotated instructions as labels. The LLM is then tasked with describing the robot's navigation trajectory based on these frames. To further encourage spatial scene understanding, we integrate the ScanQA~\citep{azuma2022scanqa} dataset, which features real-world 3D scan QA pairs involving human-edited questions and free-form answers grounded to 3D objects within each scene. For training, we utilize the multi-view RGB images from the raw scans to support this task.

Finally, to maintain the model's general capabilities, we include general video/image VQA datasets from ~\citep{liu2024improved, chen2023sharegpt4v, maaz2023videochatgpt}. This comprehensive dataset design enables \method to generalize effectively to novel scenes and real-world environments.


\myparagraph{Training and Inference Paradigm.}
Our training process begins with the stage two model of VILA, which has already undergone visual language corpus pre-training. We then apply our SFT data blend to train the entire VLM for one epoch, following standard practices. During this training, all three components—vision encoder, connector, and LLM—are unfrozen.
For the inference phase, we implement a regular expression parser~\citep{kearns1991extending}, to extract action types (such as forward or turn left) and their corresponding arguments (like specific distance or angles) from the LLM output. This method has demonstrated effectiveness in both simulated environments and real-world experiments, where we empirically found that all actions throughout all experiments are successfully matched and mapped.


\begin{figure}[t]
  \centering
  \includegraphics[width=1.0\textwidth]{images/obs_avoid_sim/LIDAR.pdf}
  \vspace{-10pt}
  \caption{Height map construction from the point cloud. (\textbf{a}) Go2 robot tracks linear and angular velocity commands while avoiding collision with obstacles in simulation. The red dots represent the LiDAR point cloud, raycasting from the sensor's center towards the terrain mesh. The left image is a preprocessed height map from the LiDAR data, with values clipped according to real-world sensor constraints. Darker colors represent lower values. (\textbf{b}) Safe robot locomotion near a transparent glass surface. The top-down height map clearly detects the glass, while the forward-facing depth and RGB images struggle to capture it.}
  \label{fig:lidar_method}
  % \vspace{-10pt}
\end{figure}

\subsection{Visual Locomotion Policy}

\label{sec:method:low}
In this section, we begin with a brief overview of the Go2 robot dog, the experimental platform used in this work. Next, we describe the development of the end-to-end vision-based control policy, which interprets high-level language navigation commands from the VLM and converts them into precise joint movements. This control policy is trained in the Isaac Sim simulator using Isaac Lab~\citep{mittal2023orbit} and then directly deployed to the real-world robot.

\myparagraph{Go2 Robot.}
As shown in Figure~\ref{fig:lidar_method}, the robot is equipped with a LiDAR sensor mounted at the base of its head, broadcasting point clouds at a frequency of 15Hz. The robot features 18 degrees of freedom (DoFs), comprising 6 DoFs for its base and 3 DoFs for each of its four legs. In the policy training process, we left the 6 DoFs on the base unconstrained so that the policy only controls the 12 joint motors on the legs.


\myparagraph{Interpreting High-level Commands}
As in our formulation, VLM outputs a fixed set of actionable words, such as \{move forward, turn left, turn right, stop\}, we casts these instructions to fixed command velocities \{$0.5 \,\si{\meter\per\second}$, $\frac{\pi}{6} \, \si{\radian\per\second}$, $-\frac{\pi}{6} \, \si{\radian\per\second}$, 0\} and execute with corresponding time durations to align with the specific VLM value.
% Need to describe how to convert the text instructions into velocities.

\myparagraph{Low-level Action and Observation Space.}
The action space $\mathbf{a}$ of the control policy is defined as the desired joint position $q^d \in \mathbb{R}^{12}$, which are converted into torque input for the simulator using the stiffness and dampness. We adopt PPO algorithm~\citep{schulman2017proximal} to train the policy. During training, the critic observes the privileged environment and generates a value function to update the actor,  while the actor only receives sensor data available in the real world. The observation space of the critic $\mathbf{o}^{c}$ contains the proprioception and velocity command at the current time step $t$ and a privileged terrain height scan around the robot. The proprioceptive data includes robot linear and angular velocity, orientation, joint positions, joint velocities, and the previous action. In the actor's observation space $\mathbf{o}^{a}$, linear velocity is excluded, as it is unavailable in the real world, and instead, a history of proprioceptive data is used to infer this information implicitly. The robot perceives the surrounding terrain using a heightmap from the LiDAR sensor.

\myparagraph{Incorporating Height Map from LiDAR Point Cloud.}
Given LiDAR's superior ability to detect transparent objects and robust performance under strong sunlight,  we chose the manufacturer-provided LiDAR as the primary sensor for perceiving the robot's surroundings and ensuring safe navigation. The Unitree L1 generates point clouds with a wide field of view of $360^{\circ}\times90^{\circ}$, from which we create a 2.5D height map based on the parameters listed in Table~\ref{tab:lidar_heightmap_settings}. For each voxel grid, the lowest value within the range is selected, and a maximum filter is then applied over the last 5 lidar point clouds to smooth the resulting height map.




\myparagraph{Training.} 
Different from most existing works~\citep{lee2020learning, miki2022learning, margolis2022rapid, lee2024learning} that utilize the two-stage teacher-student training paradigm, we adopt a single-stage manner to train the locomotion policy. Compared to two-stage training, single-stage RL is more time-efficient as it eliminates the need for policy distillation. Additionally, the policy interacts directly with the environment, allowing it to explore and potentially discover novel strategies. With the support of ray-casting in Isaac Lab, our vision-based RL policy training achieves a high throughput over 60K FPS on an RTX 4090 GPU. Training details are included in Appx.~\ref{sup:policy-details}.




==> tables/real_eval_T1.tex <==
\begin{table*}[!t]
\small
\centering
\setlength{\tabcolsep}{5.pt}
\caption{\label{tab:real_eval}Real-world experiments on humanoid (Booster T1) conducted in three environments (\texttt{Workspace}, \texttt{Home}, and \texttt{Outdoor}). Simple and Complex refer to simple and complex instruction-following tasks, respectively.}
% \vspace{-0.6em}
\scalebox{0.97}{
{\fontsize{8pt}{9pt}\selectfont
\begin{tabular}{l l cccc cccc cccc}
\toprule
& & \multicolumn{4}{c}{\texttt{Workspace}} & \multicolumn{4}{c}{\texttt{Home}} & \multicolumn{4}{c}{\texttt{Outdoor}} \\
\cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
& & \multicolumn{2}{c}{Simple} & \multicolumn{2}{c}{Complex} & \multicolumn{2}{c}{Simple} & \multicolumn{2}{c}{Complex} & \multicolumn{2}{c}{Simple} & \multicolumn{2}{c}{Complex} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14}
& & NE$\downarrow$ & SR$\uparrow$ & NE$\downarrow$ & SR$\uparrow$ & NE$\downarrow$ & SR$\uparrow$ & NE$\downarrow$ & SR$\uparrow$ & NE$\downarrow$ & SR$\uparrow$ & NE$\downarrow$ & SR$\uparrow$ \\ 
\midrule
GPT-4o~\citep{openai2024gpt4o} & & 2.01 & \underline{0.67} & 2.38 & 0.33 & \underline{1.49} & \underline{0.53} & 3.00 & 0.00 & - & \underline{0.67} & - & \underline{0.50} \\
\midrule
\method(w/o Human Videos) & & \underline{2.00} & 0.60 & \underline{1.81} & \underline{0.73} & 2.17 & 0.47 & \underline{2.32} & \underline{0.40} & - & 0.00 & - & 0.00 \\
\rowcolor{myblue}
\method & & \textbf{1.29} & \textbf{1.00} & \textbf{1.76} & \textbf{0.80} & \textbf{1.15} & \textbf{1.00} & \textbf{1.76} & \textbf{0.67} & \textbf{-} & \textbf{1.00} & \textbf{-} & \textbf{0.83} \\ 
\bottomrule
\end{tabular}
}
}

% \vspace{-10pt}
\end{table*}

